An information field theory approach to Bayesian state and parameter estimation in dynamical systems

Dynamical system state estimation and parameter calibration problems are ubiquitous across science and engineering. Bayesian approaches to the problem are the gold standard as they allow for the quantification of uncertainties and enable the seamless fusion of different experimental modalities. When the dynamics are discrete and stochastic, one may employ powerful techniques such as Kalman, particle, or variational filters. Practitioners commonly apply these methods to continuous-time, deterministic dynamical systems after discretizing the dynamics and introducing fictitious transition probabilities. However, approaches based on time-discretization suffer from the curse of dimensionality since the number of random variables grows linearly with the number of time-steps. Furthermore, the introduction of fictitious transition probabilities is an unsatisfactory solution because it increases the number of model parameters and may lead to inference bias. To address these drawbacks, the objective of this paper is to develop a scalable Bayesian approach to state and parameter estimation suitable for continuous-time, deterministic dynamical systems. Our methodology builds upon information field theory. Specifically, we construct a physics-informed prior probability measure on the function space of system responses so that functions that satisfy the physics are more likely. This prior allows us to quantify model form errors. We connect the system's response to observations through a probabilistic model of the measurement process. The joint posterior over the system responses and all parameters is given by Bayes' rule. To approximate the intractable posterior, we develop a stochastic variational inference algorithm. In summary, the developed methodology offers a powerful framework for Bayesian estimation in dynamical systems.

==> section-ift_background.tex <==
\section{Background on information field theory}
\label{sec:ift_backgound}

\newcommand{\by}{\mathbf{y}}

Information field theory is a Bayesian statistical field theory that summarizes what we know about a physical field through Bayesian inversion. 
The objective is to reconstruct a function from measurement data. 
Without loss of generality we are going to work with a scalar field $x$ that is a function of time $t$.
We write $x(t)$ for the value of $x$ at time $t$.
IFT's program starts by encoding our prior knowledge about the unknown field $x$.
This is essentially a probability measure over the function space in which $x$ lives.
Formally, we denote this probability measure with a prior ``probability density'' $p(x)$.
However, it is more convenient to work with the so-called prior information Hamiltonian of the field, which is defined up to an additive constant by:
\begin{align}
  H[x] = -\log p(x) + \text{const}.
\label{prior_ih_x}  
\end{align}
In the notation above the use of square brackets indicates that $H$ is a functional.
One thinks of the information Hamiltonian as some sort of field energy.
Fields with lower energy are more probable.

The case of a Gaussian process prior is the most common.
Suppose, for example, that the field $x$ follows a Gaussian process with a mean function $\E{x(t)} = m(t)$ and a covariance function $\C{x(t)}{x(t')} = C(t,t')$.
We write this statement in the shorthand notation:
$$
x \sim \mathcal{N}(m,C),
$$
or, in terms, of field ``probability density:''
$$
p(x) = \mathcal{N}(x|m,C).
$$
To write the information Hamiltonian, we first need to define the inverse $C^{-1}$ of the covariance function $C$.
The defining equation is:
$$
\int dt' C(t,t')C^{-1}(t',t'') = \delta(t-t'').
$$
Ignoring the normalization constant, we can write formally:
$$
p(x) \propto \exp\left\{-\frac{1}{2}\iint dt dt'\: \left[x(t)-m(t)\right]C^{-1}(t,t')\left[x(t') - m(t')\right]\right\},
$$
The reader should observe the similarities of the equation above with the probability density of a multivariate normal.
The vectors become functions, the covariance matrix and its inverse become the covariance function and its inverse, while summations become integrals.
The corresponding prior information Hamiltonian is the quadratic form:
$$
H[x] = \frac{1}{2}\iint dt dt'\: \left[x(t)-m(t)\right]C^{-1}(t,t')\left[x(t') - m(t')\right].
$$

We now discuss the normalization constant of $p(x)$ and we introduce the concept of path integrals.
The connection between $p(x)$ and the information Hamiltonian $H[x]$ can be rewritten as:
$$
p(x) = \frac{e^{-H[x]}}{Z},
$$
where $Z$ is there for normalization purposes.
Physicists call $Z$ the ``partition function.''
It is defined by:
$$
Z = \int \mathcal{D}x\: e^{-H[x]}.
$$
The integral defining $Z$ is a path integral.
It integrates over all possible fields $x$.
In other words, it integrates over a function space.
This is why another common name for this type of integral is ``functional integral.''

Note that the partition function is typically infinite.
This is the reason behind using quotes when referring to $p(x)$ as a ``probability density.''
However, this infinity does not cause problems in IFT.
First, one mostly works with the information Hamiltonian $H[x]$ which is always well-defined.
The partition function is not required to characterize either the field prior or the field posterior.
Second, when we have a parameterized prior (a case we will discuss later) we also do not need the partition function directly.
What we need is the gradient of the partition function with respect to the parameters, a quantity that is also well-defined.
Third, the infinity of $Z$ arises from the fact that we integrate over all fields.
This integration includes fields with exceedingly small scales.
When one restricts the function space so that these exceedingly small scales are removed the partition function becomes finite.

Suppose we observe some data $y$.
The likelihood function $p(y|x)$ models the measurement process.
The likelihood is the probability density of measuring $y$ when the underlying state trajectory is $x$.
The data depend on the trajectory via the action of a, not necessarily linear, measurement operator $R$, i.e.,
$p(y|x) = p(y|Rx)$.
It is more convenient to work with the data Hamiltonian, i.e., the negative logarithm of the likelihood:
$$
H(y|x) = -\log p(y|Rx) + \text{const}.
$$
Observe that this time we use parentheses instead of brackets, because $H(y|x)$ is just a multivariate function of $y$.

To give a concrete example, let us elaborate on the case of independent Gaussian measurements.
Suppose $y=(y_1,\dots,y_{n_d})$ and that the $y_i$'s are independent measurements.
The likelihood factorizes as $p(y|Rx) = \prod_{i=1}^{n_d}p(y_i|R_ix)$.
Consequently the data Hamiltonian can be written as the sum:
$$
H(y|x) = \sum_{i=1}^{n_d}\ell(y_i|R_ix),
$$
where $\ell(y_i|R_ix) = -\log p(y_i|R_ix)$ up to an additive constant.
If we assume that our measurements are scalars and normally distributed about $R_ix$ with measurement variance $\sigma_i^2$, then:
$$
\ell(y_i|R_ix) = \frac{1}{2\sigma_i^2}(y_i - R_ix)^2.
$$
In terms of the complete data Hamiltonian:
$$
H(y|x) = \frac{1}{2}(y-Rx)^T\Sigma^{-1}(y-Rx),
$$
where $\Sigma = \operatorname{diag}(\sigma_1^2,\dots,\sigma_{n_d}^2)$.

The posterior over the state trajectories $x$ conditioned on $y$ summarizes our state of knowledge about the field after seeing the data.
It can be obtained formally by applying Bayes' rule:
\begin{align*}
    p(x | y) = 
    \frac{p(y|x)p(x)}{p(y)}.
\end{align*}
In IFT, instead of the posterior probability density, we work with the posterior information Hamiltonian:
\begin{align}
   H[x|y] = -\log p(x|y) = H(y|x) + H[x] - \log Z . 
   \label{post_ih_x}
\end{align}
In this particular example, the logarithm of the partition function, $\log Z$, can be dropped from the posterior information Hamiltonian without losing anything.
It is just a constant.
However, as we will see in subsequent sections, $\log Z$ cannot be ignored if one wants to estimate any missing parameters of the prior Hamiltonian.

Returning to our concrete example (Gaussian process prior, Gaussian measurement noise) we get the following posterior information Hamiltonian (up to an additive constant):
$$
H[x|y] = \frac{1}{2}(y-Rx)^T\Sigma^{-1}(y-Rx) + \frac{1}{2}\iint dt dt'\: \left[x(t)-m(t)\right]^TC^{-1}(t,t')\left[x(t') - m(t')\right].
$$
As shown in \citep{alberts2023physics}, if $R$ is a linear operator, this posterior Hamiltonian is also a quadratic form.
As a result, the corresponding posterior field is a Gaussian process.
Furthermore, in the special case in which the operators $R_i$ sample the trajectory at different times, e.g., $R_ix = x(t_i)$ for some times $t_i$, one recovers the usual Gaussian process regression formulas \citep{rasmussen2003gaussian}.


